Tracking Amendments to Legislation and Other Political Texts with a Novel Minimum-Edit-Distance Algorithm: DocuToads

Political scientists often find themselves tracking amendments to political texts. As different actors weigh in, texts change as they are drafted and redrafted, reflecting political preferences and power. This study provides a novel solution to the prob- lem of detecting amendments to political text based upon minimum edit distances. We demonstrate the usefulness of two language-insensitive, transparent, and efficient minimum-edit-distance algorithms suited for the task. These algorithms are capable of providing an account of the types (insertions, deletions, substitutions, and trans- positions) and substantive amount of amendments made between version of texts. To illustrate the usefulness and efficiency of the approach we replicate two existing stud- ies from the field of legislative studies. Our results demonstrate that minimum edit distance methods can produce superior measures of text amendments to hand-coded efforts in a fraction of the time and resource costs.

==> backtrace_table.tex <==
\begin{table}[htpb]
\centering
\caption{Illustration of backtrace}
\begin{tabular}{c|c|c|c|c}
\textbf{$S_{1}$ index} & \textbf{$S_{2}$ index} & \textbf{Edit operation} & \textbf{$S_{1}$ word} & \textbf{$s_{2}$ word}\\
\hline
375 & 440 & & Whereas & Whereas\\
376 & 441 & &the& the\\
377 & 442 & &European &European\\
378 & 443 & &Community & Community\\
379 & 444 & Substitution & can & is\\
379 & 445 & Addition & &in\\
379 & 446 & Addition & &a\\
379 & 447 & Addition & &position\\
379 & 448 & Addition & &to\\
380 & 449 & & make & make\\
381 & 450 & & a& a\\
381 & 451 & Addition& & major\\
382 & 452 & & contribution & contribution\\
383 & 453 & & towards& towards\\
384 & 454 & & the & the\\
385 & 455 & & organisation& organisation\\
386 & 456 & & of & of
\label{tab:backtrace}
\end{tabular}
\end{table}

==> table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}\\
                    &\multicolumn{1}{c}{DocuToads MED}\\
\hline
Levenshtein MED     &       0.937\sym{***}\\
                    &    (384.15)         \\
[1em]
Constant            &       13.91\sym{**} \\
                    &      (2.78)         \\
\hline
Observations        &        2010         \\
\hline\hline
\multicolumn{2}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
